Belief-selective Propagation Detection for MIMO Systems

Compared to the linear MIMO detectors, the Belief Propagation (BP) detector has shown greater capabilities in achieving near optimal performance and better nature to iteratively cooperate with channel decoders. Aiming at real applications, recent works mainly fall into the category of reducing the complexity by simplified calculations, at the expense of performance sacrifice. However, the complexity is still unsatisfactory with exponentially increasing complexity or required exponentiation operations. Furthermore, due to the inherent loopy structure, the existing BP detectors persistently encounter error floor in high signal-to-noise ratio (SNR) region, which becomes even worse with calculation approximation. This work aims at a revised BP detector, named {Belief-selective Propagation (BsP)} detector by selectively utilizing the \emph{trusted} incoming messages with sufficiently large \textit{a priori} probabilities for updates. Two proposed strategies: symbol-based truncation (ST) and edge-based simplification (ES) squeeze the complexity (orders lower than the Original-BP), while greatly relieving the error floor issue over a wide range of antenna and modulation combinations. For the $16$-QAM $8 \times 4$ MIMO system, the $\mathcal{B}(1,1)$ {BsP} detector achieves more than $4$\,dB performance gain (@$\text{BER}=10^{-4}$) with roughly $4$ orders lower complexity than the Original-BP detector. Trade-off between performance and complexity towards different application requirement can be conveniently obtained by configuring the ST and ES parameters.

==> 1.intro.tex <==
	\section{Introduction}
	\IEEEPARstart{T}{hanks} to its high spatial efficiency (SE), improved energy efficiency (EE), and increased data transmission rate \cite{Rusek13_SPM, larsson14_CM, lu14_JSTSP},
multiple-input and multiple-output (MIMO) has been one of the key technologies in 5G and beyond 5G (B5G) wireless communication systems. Although the MIMO systems can enjoy both diversity gain and multiplexing gain compared with the conventional single-input single-output (SISO) systems, the signal detection of the MIMO systems suffer from a relatively higher computational complexity.

MIMO detection is one of the main bottlenecks in terms of the application for the realistic MIMO systems. The intention of the MIMO detection is to recover the transmitted signal from the observation of the receiver, under the knowledge of the channel state information (CSI). Due to the finite set mapping of the transferred symbols in MIMO systems, the detection problem is actually an NP-hard \cite{Fincke85_MC} problem. The complexity of the MIMO detection problem increases with the scale of the antenna arrays in the systems. And MIMO detection algorithms are investigated in many years \cite{Yang15_CSTO, Albeem19_CSTO}.

Trade-off between low complexity and good performance is always an important issue in MIMO detection.
\textit{Maximum likelihood} (ML) or \textit{maximum a posterior} (MAP) detection enumerates all probabilities of the transmitted symbols, which achieves optimal performance. However, the exhaustive search causes prohibitive complexity in MIMO systems.
Linear MIMO detections, e.g., zero-forcing (ZF)\cite{Spencer04_TSP}, linear minimum mean square error (LMMSE) \cite{Kim08_TWC},
and linear iterative algorithms, e.g., successive over relaxation (SOR) \cite{Gao14_GlobalCom}, Gauss-Seidel (GS) \cite{Dai15_TVT}, and coordinate desent (CD) \cite{Studer16_TCASI},
hold on low implementation complexity but suffering from unsatisfactory performance under realistic propagation condition channel.
Inference cancellation based nonlinear detection algorithms such as MMSE successive interference cancellation (MMSE-SIC) \cite{Luo07_TWC}, MMSE based parallel interference cancellation (MMSE-PIC) \cite{Studer11_JSSC}, achieves near-optimal performance but with respect to higher complexity compared to linear algorithms. Sphere decoding (SD) \cite{Brink03_TCOM} and K-best \cite{Guo06_JSAC} methods are alternative suboptimal nonlinear detection algorithms based on tree search, which still endure unacceptable computational complexity for large-scale MIMO systems.

Message passing detection algorithms are extensively investigated in recent years thanks to its stronger robustness character, lower complexity and better performance compared with the conventional detection algorithms.
Approximate message passing (AMP) \cite{Donoho09_PNAS, Montanari10_ITW_I, Montanari10_ITW_II, Montanari11_TIT} was initially proposed to recover the sparse signal and then used in MIMO detection \cite{Wu14_JSTSP, Jeon15_ISIT}.
The following works about AMP include generalized AMP (GAMP) \cite{Rangan11_ISIT}, orthogonal AMP (OAMP) \cite{Junjie17_ACCESS}, and vector AMP (VAMP) \cite{Rangan19_TIT}. The AMP based data detection algorithms retain low complexity since they only need to compute matrix-vector multiplication in each iteration.
Expectation propagation (EP) is an alternative message passing detection algorithm \cite{Javier14_TCOM} with a proven ability of achieving optimal performance \cite{Takeuchi20_TIT}, thus has been widely investigated recently \cite{Tan19_TVT, Tan20_TCASII, Yao21_TCOM}.
However, AMP and GAMP only achieve near-optimal performance with respect to Gaussian independent identical distributions (i.i.d) channel coefficients.
The VAMP and EP detection algorithms rely on large-scale MIMO dimension limit and compression rate threshold \cite{Takeuchi20_TIT} to exhibit an excellent performance. In addition, the complexity of the EP detection is relatively unsatisfactory, which limits its application in realistic MIMO systems.

Another type of message passing detection is belief propagation (BP) algorithm \cite{pearl1988probabilistic, Kschischang01_TIT}, which has been widely investigated as decoding algorithm in channel codes such as low density parity check (LDPC) codes \cite{Jinghu05_TCOM, Declercq07_TCOM} and polar codes \cite{Arikan08_CML, Yuan14_TSP, Shen20_TCOM}.
Although it may be not optimal because of the loopy factor graphs \cite{yedidia2003understanding} with respect to dense channel matrix, it is indicated empirically that the BP algorithms is always exhibiting an satisfactory results in real systems.
In fact, rather than the intention of achieving channel capacity performance, what we are interested is an algorithm of unified graphical framework and strong robustness in a 5G/B5G wireless system.
The authors in \cite{Haroun14_WCNC, Narasimhan14_VTC, Jing17_ASICON} show that BP-based iterative detection and decoding (IDD) systems can obtain a good enough performance.
Besides, the graph representation algorithm can be more friendly to hardware design and implementation.
The authors in \cite{Jun08_JSAC} show that BP detection is still feasible when a MIMO system contains smaller number of receive antennas than that of the transmit antennas, and its performance is also satisfactory under the frequency-flat and frequency-selective fading channels.

Reviewing BP algorithm in MIMO detection, the main investigation lies in the following aspects:
1) Elimination of circles \cite{Jacob11_TIT, Yoon14_TVT}, 2) acceleration of convergence \cite{murphy1999loopy, Pritam10_ITW, Junmei15_SiPS, Su15_TSP, yang2018low}, and 3) reduction of complexity \cite{Jun08_JSAC, Feichi11_SS, Pritam11_JSTSP, Yaping17_WCSP}.
The authors in \cite{Jacob11_TIT, Yoon14_TVT} transform the conventional factor graphs into the cycle-free graphs, thus enjoying a good performance.
The authors in \cite{murphy1999loopy, Pritam10_ITW, Junmei15_SiPS, Su15_TSP, yang2018low} utilize factor damping techniques to accelerate the convergence rate, which also improves symbol error rate (SER) performance.
The straightforward full-edge BP (FE-BP) detection suffers from the same complexity as the ML detection, because of the computation of the marginal probability of the factor nodes. In \cite{Jun08_JSAC}, the authors proposed a edge-based regular-$d_f$ (EBRDF) BP detection
with respect to pruned graphical models in which each factor node only remains $d_f$ dynamic edges. The authors in \cite{Feichi11_SS, Pritam11_JSTSP, Yaping17_WCSP} further reduce the computational complexity by approximating the neighbors of each edge with a Gaussian distribution. However, the Gaussian approximation only works when the antenna size is large enough to meet the central limit theorem.

In this paper, a novel complexity-reduced BP detection algorithm is proposed, which we call it extend min-sum BP (EMS-BP) detection.
The EMS scheme proposed by Declercq \cite{Declercq05_ISIT, Declercq07_TCOM} is originally used to achieve a low complexity for decoding of nonbinary LDPC (NB-LDPC) codes. Then Voicila and Declercq further present the extension of EMS for the high order fields \cite{Declercq10_TCOM}. The EMS strategy in the decoding of the NB-LDPC codes is different from that in the MIMO BP detection, because the check matrix of the NB-LDPC is sparse and over GF($q$), while the coefficients in the channel matrix are dense and random.
However, we can still take advantage of the EMS scheme in the MIMO BP detection to reduce the computational complexity, since the graphical models and the search space of the MIMO BP detection is consistent with that of the NB-LDPC codes.
The main contributions of this work are listed as follows:
\begin{itemize}
  \item The EMS-BP MIMO detection algorithm is proposed.
  \item The EMS-BP MIMO detection algorithm is proposed.
  \item The EMS-BP MIMO detection algorithm is proposed.
\end{itemize}



%Because the goal of the EMS is not the optimal solution of the NB-LDPC codes, but the sub-optimal results with a considerably low complexity, the EMS algorithm only remains $n_m$ largest log-likelihood ratio (LLR) values from $q$ LLR values ($1\leq n_m\leq q$) with respect to the messages transmitted from the symbol nodes to the factor nodes.

%Since the factor graph of NB-LDPC codes is consistent with that of the MIMO detection, therefore, we can take advantage of the EMS scheme in the MIMO BP detection, in order to a decreased computational complexity. It is of worthy to note that the EMS strategy in the decoding of the NB-LDPC codes is different from that in the MIMO BP detection, because the check matrix of the NB-LDPC is sparse and over GF($q$), while the coefficients in the channel matrix are dense and random. The detailed discussion of the EMS-BP in MIMO detection can be found in Sec.~III.





%The factor graph of BP detection is constructed with the channel matrix $\mathbf{H}$, thus containing $N$ observation nodes (ON) representing the receive signals, and $M$ symbol nodes (SN) with respect to the hidden transmitted data.



%The conventional message passing detection is belief propagation based on graphical models.



	

